FASTER: A Font-Agnostic Scene Text Editing and Rendering Framework

Scene Text Editing (STE) is a challenging research problem, that primarily aims towards modifying existing texts in an image while preserving the background and the font style of the original text. Despite its utility in numerous real-world applications, existing style-transfer-based approaches have shown sub-par editing performance due to (1) complex image backgrounds, (2) diverse font attributes, and (3) varying word lengths within the text. To address such limitations, in this paper, we propose a novel font-agnostic scene text editing and rendering framework, named FASTER, for simultaneously generating text in arbitrary styles and locations while preserving a natural and realistic appearance and structure. A combined fusion of target mask generation and style transfer units, with a cascaded self-attention mechanism has been proposed to focus on multi-level text region edits to handle varying word lengths. Extensive evaluation on a real-world database with further subjective human evaluation study indicates the superiority of FASTER in both scene text editing and rendering tasks, in terms of model performance and efficiency. Our code will be released upon acceptance.

==> sec/5_limitations.tex <==
\section{Limitations}\label{sec:limitations}
The proposed STE in the passage has a limitation: it relies on mask guidance maps to identify editing regions explicitly. While this filtering helps eliminate background distractions and guides the network to focus on editing rules for text regions, challenges may arise with complex or irregular text layouts. The structure guidance maps assume well-defined masks for text regions, which may be limiting when dealing with diverse text forms like handwritten, distorted, or overlapping text. Generating accurate mask guidance maps in such cases can be challenging, potentially leading to errors or inconsistencies during the editing process.
% In Figure~\ref{fig:vis_3} we have shown some failure cases of our method.


